RePr: Improved Training of Convolutional Filters

A well-trained Convolutional Neural Network can easily be pruned without significant loss of performance. This is because of unnecessary overlap in the features captured by the network's filters. Innovations in network architecture such as skip/dense connections and Inception units have mitigated this problem to some extent, but these improvements come with increased computation and memory requirements at run-time. We attempt to address this problem from another angle - not by changing the network structure but by altering the training method. We show that by temporarily pruning and then restoring a subset of the model's filters, and repeating this process cyclically, overlap in the learned features is reduced, producing improved generalization. We show that the existing model-pruning criteria are not optimal for selecting filters to prune in this context and introduce inter-filter orthogonality as the ranking criteria to determine under-expressive filters. Our method is applicable both to vanilla convolutional networks and more complex modern architectures, and improves the performance across a variety of tasks, especially when applied to smaller networks.

==> figures/related_works.tex <==
We have divided the discussion of related works into categories that broadly cover our area of research.

\textbf{Training Scheme}
Many changes to the training paradigm have been proposed to reduce over-fitting and improve generalization.
Dropout~\cite{Wu2015TowardsDT} is widely used in training deep nets. 
By stochastically dropping the neurons it prevents co-adaption of feature detectors.
A similar effect can be achieved by dropping subset of activations ~\cite{Wan2013RegularizationON}.
Wu \etal~\cite{Wu2015TowardsDT} extend the idea of stochastic dropping to convolutional neural networks by probabilistic pooling of convolution activations.
Yet another form of stochastic training recommends randomly dropping entire layers~\cite{Huang2016DeepNW}. 
This forces the model to learn similar features across various layers which prevent extreme overfitting.
On the contrary, our technique encourages the model to learn to use a linear combination of features instead of duplicating the same feature.



\textbf{Model Compression}
Knowledge Distillation (KD)~\cite{Hinton2015DistillingTK} is a training scheme which uses soft logits from a bigger capacity trained model (teacher) to train a smaller model (student).
Soft logits capture hierarchical information about the object and provides a more smooth loss function for the optimization. This leads to easier training and better convergence for small models.
Stronger forms of KD where a model matches intermediate activations have also been proposed~\cite{Romero2014FitNetsHF}. 
By forcing the student model to match the output statistics from the teacher, it provides the directions for weight updates which are not found in the gradients.
In a surprising result, Born-Again-Network~\cite{Furlanello2018BornAN} shows that if the student model is of the same capacity as the teacher it can outperform the teacher.
All forms of KD requires another well-trained teacher and added training cost. 
Our training scheme does not depend on an external teacher and requires less training than KD. More importantly, our scheme is complementary to KD. 
When combined with KD, our method gives better performance than can be achieved by either technique independently. 
We discuss this in detail in the section~\ref{lbl:distillation}.


\textbf{Neuron ranking}
Interest in finding the least salient neurons/weights has a long history. 
LeCun~\cite{LeCun1989OptimalBD} and Hassibi\etal~\cite{Hassibi1992SecondOD} show that using Hessian, which contains second-order derivative, identifies the weak neurons and performs better than using the magnitude of the weights.
In the advent of deep networks, computing the Hessian is expensive and thus is not popular as a choice of neuron selectivity.
Han \etal~\cite{Han2015DeepCC} show that the norm of weights is still an effective ranking criteria and yields sparse models.
The sparse models do not translate to faster inference, but as a neuron ranking criteria they are effective.
Computing the norm of the weights is easy and data-free, thus lends itself to pruning for transfer learning.
Hu \etal~\cite{Hu2016NetworkTA} explore use of activations for filter ranking. 
They measure the Average Percentage of Zeros (APoZ) in the activations and use a data-driven threshold to determine the cut-off. 
It is a useful comparison metric and works well when the training data is available.
ThinNet~\cite{Luo2017ThiNetAF} explores reconstruction error between the layers, thus does not lead to a generalized filter ranking criteria.
Molchanov \etal~\cite{Molchanov2016PruningCN} recommend second term from the Taylor expansion of the loss function, which is a product of activation and the gradient.
Currently, it is the state-of-the-art in filter pruning and works well for transfer pruning.
Our filter ranking criteria, \textit{inter}-filter orthogonality, is yet another approach and is designed especially for the purposes of temporary pruning. 
We provide detail comparison with these metrics in the section~\ref{sec:metric} and show results on using these metrics with our training scheme.


\textbf{Feature correlation}
A well-known shortcoming of vanilla convolutional networks is their correlated feature maps~\cite{Cogswell2015ReducingOI, Glorot2010UnderstandingTD}.
Architectures like Inception-Net~\cite{Szegedy2015GoingDW} are motivated by analyzing the correlation statistics of features across layers.
Szegedy \etal claims that a network-in-network block which produces concatenated features from various sized filters reduces the correlation between the layers.
However, correlation of singular values across inception layers show that there are a significant overlap of activations~\cite{Raghu2017SVCCASV}. 
More recent architectures like DenseNet also claim to implicitly reduce feature correlations. 
The dense connections, which concatenate activations from previous layers, reduces the need to learn the same features~\cite{Huang2017DenselyCC}.
That said, DenseNets are computationally expensive and require large memory to store all previous activations.
Our aim is to induce decorrelated features without changing the architecture of the convolutional network.
This benefits all the existing implementations of ConvNet without having to change the infrastructure.
While our technique performs best with vanilla ConvNet architectures it still marginally improves performance of modern architectures.

Chen \etal ~\cite{Chen2017TrainingGO} used privileged information, like segmentation maps, to encourage diversity in feature maps, and approximate group orthogonal filters.
Unfortunately, such techniques restrict themselves to domains where segmentation maps are available for the task of image classification. 
Our method does not rely on any external information or a pretrained model.

\textbf{Architecture Search} 
It is possible to argue that works neural architecture search ~\cite{Liu2017ProgressiveNA, Real2018RegularizedEF, Zoph2016NeuralAS} is related to our technique. 
In essence, they also change network architecture during training and are free to explore more extreme versions of the structure, while our training regime restricts itself to the original architecture. Our scheme is trying to find better weights given a fixed architecture and this is a fundamental distinction with architecture search.
Potential for finding a better generalizing architecture diminishes by restricting to a fixed final architecture but asserts itself to several applications where predetermined architecture is warranted.
This could be due to certified model deployment, memory requirements or better interpretability of simpler ConvNets.
